SCITAT: A Question Answering Benchmark for Scientific Tables and Text Covering Diverse Reasoning Types

Scientific question answering (SQA) is an important task aimed at answering questions based on papers. However, current SQA datasets have limited reasoning types and neglect the relevance between tables and text, creating a significant gap with real scenarios. To address these challenges, we propose a QA benchmark for scientific tables and text with diverse reasoning types (SciTaT). To cover more reasoning types, we summarize various reasoning types from real-world questions. To involve both tables and text, we require the questions to incorporate tables and text as much as possible. Based on SciTaT, we propose a strong baseline (CaR), which combines various reasoning methods to address different reasoning types and process tables and text at the same time. CaR brings average improvements of 12.9% over other baselines on SciTaT, validating its effectiveness. Error analysis reveals the challenges of SciTaT, such as complex numerical calculations and domain knowledge.

==> old_version/1.introduction_1216.tex <==
% SciQA任务，引出学术领域的TATQA任务
% SciQA是自然语言处理的一项重要的任务，指根据学术领域的文献、论文或数据，解决用户提出的学术相关的问题
Scientific Question Answering (SQA) is an essential task for addressing questions raised by researchers based on scientific papers \cite{tsatsaronis2015overview-BIOASQ,pmlr-v202-QASA}.
% 推动学术问答的发展能够增加学术资源的可访问性，加速知识获取，在科研、教育等场景中有着广泛的应用
Promoting the development of SQA can accelerate the acquisition of knowledge \cite{taylor2022galactica,ai4science2023Scientific-Discovery}.
% 尤其是论文中通常包含着密集的专业术语和异构的知识表示，这为学术QA带来了挑战
In particular, scientific papers usually contain dense technical terms and heterogeneous data representations, which brings challenges to SQA \cite{pramanick2024spiqa}.


% 动机，前人工作不足
% 为了更好地评测和增强模型学术QA的能力，前人提出了很多学术QA数据集
To evaluate and enhance the model capabilities in SQA, numerous datasets are proposed \cite{pampari-etal-2018-emrqa,pappas-etal-2020-biomrc,jin-etal-2019-pubmedqa}.
% 然而，现有的工作存在以下不足
However, existing datasets exhibit the following limitations, as shown in Table~\ref{tab:comparison_sciqa}. 
% 并且，前人的推理的类型较为局限，且和真实场景有较大差距。
Firstly, the \textbf{reasoning types are relatively narrow}, failing to capture the complexity of real scenarios, such as data analysis, which is frequently encountered in actual queries.
% 要么只关注文本，要么只关注表格
Secondly, prior works \textbf{focus only on split text and tables} \cite{pmlr-v202-QASA,moosavi2021scigen,pramanick2024spiqa}, overlooking the relevance between tables and text, thereby limiting their applicability \cite{chen-etal-2020-hybridqa,wang2022hybridqa-survey}.
% 然而，现有学术QA数据集大部分只关注了对论文中文本的理解和推理，忽略了论文中经常出现的表格
% However, most existing scientific QA datasets primarily focus on understanding and reasoning over textual content, overlooking the tables that frequently appear in papers.
% 而SciGen, SciTab和SPIQA考虑到了学术论文中表格的问答，但忽略了表格和文本的链接，造成其应用场景有限
% While datasets such as SciGen~\cite{moosavi2021scigen}, SciTab~\cite{lu-etal-2023-scitab}, and SPIQA~\cite{pramanick2024spiqa} incorporate QA tasks involving tables in papers, they fail to account for the links between tables and text, thereby limiting their applicability in real-world scenarios \cite{chen-etal-2020-hybridqa,wang2022hybridqa-survey}.
% 并且，前人工作没有针对学术领域在表格和文本上的问答任务的知识密集和数值密集的特点设计方法，导致在这些数据集上的提升有限
% Moreover, previous works have not designed methods tailored to address the knowledge- and numerically-intensive nature of the SQA task, leading to limited performance improvements \cite{moosavi2021scigen,lu-etal-2023-scitab,pramanick2024spiqa}.
To address the limitations, in this paper:
% 所以，本文提出一个学术QA数据集,同时考虑文本和表格信息
\textit{(i)} We introduce a new SQA benchmark, covering diverse real-scenery reasoning types and considering tables and text simultaneously.
% 为了增强数据集上的性能，我们提出我们的方法，which增强模型在多种推理类型上的性能，并且同时处理文本和表格的能力
\textit{(ii)} To enhance the performance on the benchmark, we propose a strong baseline, which is capable of handling multiple reasoning types and processing tables and text simultaneously.
% \textit{(ii)} To enhance performance on the benchmark, we propose \ourmethod method, which enhances the model capability to handle multiple reasoning types and process tables and text concurrently.



% % 为了更好地评测和增强模型学术QA的能力，前人提出了很多学术QA数据集
% To better evaluate and enhance the model ability of scientific QA, many scientific QA datasets are proposed.
% % 然而，现有学术QA数据集大部分只关注了对论文中文本的理解和推理，忽略了论文中经常出现的表格
% However, most scientific QA datasets only focus on the text in the paper, ignoring the tables in the papers.
% % 所以，一些工作提出了关于论文中表格的问答，如表1中总结。
% Therefore, some works propose datasets that require reasoning on the scientific tables, as summarized in Table 1.
% % 比如，SciGen关注于生成表格相关的描述，SciTab关注于表格的事实验证任务（SPIQA关注于关于表格的问答）
% For example, SciGen~\cite{moosavi2021scigen} concentrates on generating table-related descriptions, and SciTab~\cite{lu-etal-2023-scitab} focuses on the table fact-verification task.
% % 然而，这些工作的推理类型比较局限，而且没有关注到表格和文本的链接，导致问题只能根据表格回答，造成其应用场景有限
% Nevertheless, the reasoning types of these works are relatively limited, and they ignore the links between the table and text \cite{chen-etal-2020-hybridqa,zhu-etal-2021-tat}, resulting in limited application scenarios.
% % 并且，前人工作没有针对学术领域TAT-QA的知识密集和数值密集的特点设计方法，导致在这些数据集上的提升有限
% In addition, previous works do not design methods for scientific QA on the tabular and textual content, resulting in limited improvement.
% % 所以，本文提出一个需要联合表格和文本问答的多推理类型的学术QA数据集，
% Therefore, we propose a QA dataset a scientific hybrid of tabular and textual content with diverse reasoning types (\ourdataset).
% % 并且，我们提出我们的方法，which结合LLM的多种推理能力，来提升模型在学术领域TAT-QA任务上的性能
% Also, we propose our method (\ourmethod), which integrates the multiple reasoning capabilities of LLM to improve the performance on \ourdataset.

\begin{figure*}
    \centering
    \includegraphics[width=.95\linewidth]{fig/intro.pdf}
    \vspace{-0.5em}
    \caption{
    % 我们数据集中四种推理形式的解释
    Illustrations of the reasoning types in \ourdataset.
    % 左边虚线框内展示了论文中的片段和表格，用颜色标注的地方为对应颜色的问题推理时需要用到的上下文
    The tables and text (left) show color-coded spans for question context.
    % ，右边的4个问题分别是4种推理形式的例子，with rationale and answer
    The questions (right) are examples of $4$ reasoning types, with their rationales and answers.
    }
    \label{fig:intro}
\end{figure*}
% \vspace{-0.5em}
% \begin{table*}[t]
%     \centering
%     \small
%     \input{tab/comparison_sciqa}
%     \caption{
%         Comparison of \ourdataset to recent SQA datasets.
%         TAT denotes Table and Text.
%     }
%     \label{tab:comparison_sciqa}
% \end{table*}


\begin{table}[t]
    \centering
    \small
    \input{tab/comparison_sciqa}
    % \vspace{-0.5em}
    \caption{
        Comparison of \ourdataset to recent SQA datasets.
        TaT denotes Table and Text.
        % \textbf{\uppercase\expandafter{\romannumeral1}}, \textbf{\uppercase\expandafter{\romannumeral2}}, \textbf{\uppercase\expandafter{\romannumeral3}}, and \textbf{\uppercase\expandafter{\romannumeral4}} denote the reasoning type of Look Up, Numerical Reasoning, Data Analysis, and Tabulation respectively. 
        \textbf{LU}, \textbf{NR}, \textbf{DA}, and \textbf{TB} denote the reasoning type of Look Up, Numerical Reasoning, Data Analysis, and Tabulation respectively. 
        The examples of the reasoning types can be seen in Figure~\ref{fig:intro}. 
        We introduce existing datasets in detail in Appendix~\ref{subsec:Comparison with Previous Scientific QA Datasets}.
    }
    \label{tab:comparison_sciqa}
\end{table}


% 数据集介绍
% 首先，我们提出全新的学术的TAT-QA数据集，标注了中英文双语的问题、rationale和答案
Firstly, we propose a QA benchmark for scientific tables and text (\ourdataset), which are collected from papers in arXiv.org.
% 我们从arxiv网站上收集了论文中的表格和文字
% We collect the text and tables from the papers in arXiv.org.
% 并且，为了贴合实际场景的学术的TAT-QA数据，我们观察了真实的用户问题，并结合前人工作对问题预先制定了分类
\textbf{To fit the actual scenario}, we summarize various reasoning types from the real questions raised by researcher (see Figure~\ref{fig:intro}).
% 我们提供段落和表格提示LLM根据分配的推理类型生成问题，并且问题需要尽量同时涉及段落和表格
\textbf{To ensure the questions involve both tables and text}, we request questions that involve both tables and text as much as possible.
% 我们还雇佣专业的标注者根据问题的要求对问题检查和修改
% We also hire professional annotators to check and refine the questions according to the requirements.
% 我们还用LLM生成了问题的推理过程和答案，同样雇佣标注者检查并修改
% We use LLM to generate the rationales and answers and also hire annotators to check and refine.
% 为了保证问题的多样性和答案的一致性，我们采用LLM生成不同类别的问题和相应的答案，并请标注者检查数据并对错误数据修改
% We prompt LLM to generate questions corresponding to different reasoning types, and their rationales and answers following previous works \cite{wu2024tablebench}.
% We also employ professional annotators to check and refine the generated data.
% 总共，我们的数据集包含来自875篇论文的975个问题
Overall, \ourdataset contains $953$ questions derived from $871$ papers.
% 为了从不同角度评测模型的能力，我们提供了两个setting：long-context，即提供整篇论文内容，以及shot-context，提供问题相关的段落和表格
% To evaluate the model capabilities from different perspectives, we provide two settings: long-context, where the entire paper is provided, and shot-context, where only the text and tables relevant to the question are provided.
% 经过数据分析可以发现，我们的数据涉及了14种问题类型，不仅需要模型能够从hybrid上下文中查找信息，进行数值计算，还需要进行复杂的数据分析和根据要求整理表格，很好地符合了现实场景用户的需求
Data analysis reveals that \ourdataset encompasses $4$ reasoning types and $13$ subtypes, covering the types summarized from the real questions in SparkRA~\cite{wu-etal-2024-sparkra} and previous works \cite{lu-etal-2023-scitab,wu2024tablebench}.
\ourdataset not only require the model to look up information and numerical reasoning but also require complex data analysis and tabulation, effectively meeting the needs of researchers in real-world scenarios.
% 并且我们的数据集同时覆盖了short-form的答案和free-form的答案，which更贴合实际场景的需求
% Furthermore, \ourdataset includes both short-form and free-form answers, which more closely align with the demands of real-world scenarios \cite{khashabi-etal-2021-gooaq-open}.


% 方法介绍
% 考虑到我们的数据集的特点，我们提出我们的方法，通过融合不同的推理方法来更好地处理科学数据
Considering the challenges of \ourdataset, we propose a strong baseline to better process scientific data by integrating reasoning methods (\ourmethod).
% 具体来说，我们将推理过程分解为Calculator和Reasoner。
% Specifically, we decompose the reasoning process into two modules: a Calculator and a Reasoner. 
% 为了处理多种推理类型，我们的方法分为Calculator和Reasoner两个模块，分别关注数值推理和文本推理
\textbf{To handle multiple reasoning types}, \ourmethod consists of two modules: Calculator and Reasoner, focusing on different reasoning types. 
% 为了同时处理文本和表格，Calculator将表格和文本中的有效的数值信息抽取出来，提供给Reasoner进行推理
\textbf{To process both tables and text}, Calculator extracts and calculates numerical information from tables and text, which is then provided to Reasoner for further reasoning.
% 我们首先提示LLM生成代码来求解回答问题需要的数值信息，再根据代码的执行结果提示LLM继续推理得到最终答案
% First, the Calculator generates the program that solves the numerical information required to answer the question. 
% Then, based on the execution results of this program, the Reasoner continues reasoning and derives the final answer, highlighting the challenges of \ourdataset.


% 实验结果
% 我们构建了一系列baseline方法，评测了闭源模型和开源模型在我们数据集上的性能
We construct a series of baselines and evaluate the performance of both closed-source and open-source models on \ourdataset. 
% 我们的方法超过最佳基线%
Experiment results reveal that \ourmethod outperforms other baselines with $12.9\%$ on average, proving its effectiveness. 
% 即使如此，gpt-4o在我们数据集上的准确率也低于50，证明我们数据集是一个有挑战的benchmark
However, the Exact Match of \ourmethod using \texttt{gpt-4o} is still below $50\%$, which demonstrates that \ourdataset serves as a challenging benchmark.
% 错误分析揭示了我们数据集的主要挑战，比如定位相关信息，正确的数值计算，以及需要领域知识等
Error analysis reveals the main challenges of \ourdataset, such as grounding the relevant context, complex numerical calculation, and the need for domain knowledge.


% 贡献
% 我们的贡献如下
Our contributions are as follows:
\begin{enumerate}
    % 1. 据我们所知，我们创建了首个scientific QA benchmark over tabular and textual data，包含多样的推理类型
    \item To the best of our knowledge, we develop \ourdataset, the first scientific QA benchmark for tables and text, covering diverse reasoning types based on real scenarios.
    % 2. 我们提出了方法，通过融合不同的推理方法来解决多种推理类型和同时处理表格和文本
    \item We propose \ourmethod, a strong baseline to solve various reasoning types and process tables and text by integrating reasoning methods.
    % 3. 实验结果表明，我们的方法相比较基线提升%证明了我们方法的有效性，但仍和人类性能有较大差距，证明了我们数据集的挑战
    \item Experimental results show that \ourmethod outperforms other baselines by $12.9\%$ on average, confirming its effectiveness.
\end{enumerate}


==> tab/case_miss.tex <==
\begin{tabular}{p{0.9\textwidth}}
\toprule
\textbf{The prompt for DirectQA} \\
\midrule
Table (including its label, caption, and content):\\
\verb!|  | SZ-All | SZ-Eco | TB | WP-All | WP-Eco | WP-Top-1 | WP-Top-3 | Zeit-All |!\\
\verb!|:---|:---|:---|:---|:---|:---|:---|:---|:---|!\\
\verb!| SZ-All | --- | \gn{1.3322676295501878e-15} | \gn{6.661338147750939e-16} | \gn{3.774758283725532e-15} | \gn{3.774758283725532e-15} | \gn{3.254679608977452e-300} | \gn{2.1646377602758511e-299} | \gn{1.4432899320127035e-15} |!\\
\verb!| SZ-Eco | --- | --- | \gn{2.1329858606811136e-05} | \gn{1.5543122344752192e-15} | \gn{1.5543122344752192e-15} | \gn{1.3322676295501878e-15} | \gn{1.3322676295501878e-15} | \gn{1.1102230246251565e-16} |!\\
\verb!| TB | --- | --- | --- | \gn{1.5543122344752192e-15} | \gn{1.5543122344752192e-15} | \gn{6.661338147750939e-16} | \gn{6.661338147750939e-16} | \gn{1.5543122344752192e-15} |!\\
\verb!| WP-All | --- | --- | --- | --- | \rn{0.3046738960267182} | \gn{9.832576356449962e-07} | \gn{0.0002125731914102147} | \gn{2.1094237467877974e-15} |!\\
\verb!| WP-Eco | --- | --- | --- | --- | --- | \gn{1.7187396805784516e-07} | \gn{6.944014693321954e-05} | \gn{2.1094237467877974e-15} |!\\
\verb!| WP-Top-1 | --- | --- | --- | --- | --- | --- | \rn{0.47749460966697926} | \gn{1.4432899320127035e-15} |!\\
\verb!| WP-Top-3 | --- | --- | --- | --- | --- | --- | --- | \gn{1.4432899320127035e-15} |!\\
\verb!| Zeit-All | --- | --- | --- | --- | --- | --- | --- | --- |!\\
Paragraph:\\
Figure \verb!\ref{fig:MinEdgeWeightVsCWS}! essentially confirms the results obtained so far.
However, we now observe, for higher $\alpha$ values, that the cluster values of textbook-based networks become seemingly indistinguishable from those observable for Wikipedia corpora-based networks -- the same observation concerns the SZ-Eco-based networks.
Textbook-based TCNs are again hardly distinguishable from TCNs derived from informal language newspaper articles about topics related to economics (SZ-Eco). 
In any case, Table \verb!\ref{tab:cws-x}! also shows that all value distributions along the x and y axis are now distinguishable with only three exceptions: the dynamics of clustering is obviously more corpus specific.\\
\\
\bottomrule
\end{tabular}
